Gromov-Witten invariants of blow-ups

In the first part of the paper, we give an explicit algorithm to compute the (genus zero) Gromov-Witten invariants of blow-ups of an arbitrary convex projective variety in some points if one knows the Gromov-Witten invariants of the original variety. In the second part, we specialize to blow-ups of P^r and show that many invariants of these blow-ups can be interpreted as numbers of rational curves on P^r having specified global multiplicities or tangent directions in the blown-up points. We give various numerical examples, including a new easy way to determine the famous multiplicity d^{-3} for d-fold coverings of rational curves on the quintic threefold, and, as an outlook, two examples of blow-ups along subvarieties, whose Gromov-Witten invariants lead to classical multisecant formulas.

==> definitions.tex <==
% Main file: latex main

\makeatletter
\def\@gw[#1]#2#3{I_{#2}^{#1}({#3})}
\def\gw{\@ifnextchar[{\@gw}{\@gw[]}}
\def\@di[#1]#2#3#4{I_{#2}^{#1}(#3\,|\,#4)}
\def\di{\@ifnextchar[{\@di}{\@di[]}}
\def\@Mb#1{\bar M(#1)}
\def\@Mbz[#1]#2{\bar M_{0,#1}(#2)}
\def\Mb{\@ifnextchar[{\@Mbz}{\@Mb}}
\def\@Mm#1{M(#1)}
\def\@Mmz[#1]#2{M_{0,#1}(#2)}
\def\Mm{\@ifnextchar[{\@Mmz}{\@Mm}}
\newcommand {\Md}[4]{\bar M_{0,#1,#2}(#3\,|\,#4)}
\newcommand {\virt}[1]{[#1]^{virt}}
\newcommand {\fund}[1]{[#1]}
\newcommand {\vdim}{\mathop {\rm vdim}\;}
\newcommand {\codim}{\mathop {\rm codim}\;}
\newcommand {\diag}{\mathop {\rm diag}\;}
\newcommand {\PGL}{\mathop {\rm PGL}\;}
\renewcommand {\min}{\mathop {\rm min}\;}
\renewcommand {\dim}{\mathop {\rm dim}\;}
\renewcommand {\deg}{\mathop {\rm deg}\;}
\renewcommand {\ker}{\mathop {\rm ker}\;}
\renewcommand {\max}{\mathop {\rm max}\;}
\renewcommand {\exp}{\mathop {\rm exp}\;}
\newcommand {\coker}{\mathop {\rm coker}\;}
\newcommand {\rk}{\mathop {\rm rk}\;}
\newcommand {\im}{\mathop {\rm im}\;}
\newcommand {\spc}{\@ifnextchar.{}{\@ifnextchar,{}{\@ifnextchar:{}{ }}}}
\newcommand {\sth}{\; \cdot \;}
\newcommand {\bX}{\tilde X}
\newcommand {\blowup}{blow-up\spc}
\newcommand {\blowups}{blow-ups\spc}
\newcommand {\gwinv}{Gromov-Witten invariant\spc}
\newcommand {\gwinvs}{Gromov-Witten invariants\spc}
\newcommand {\nonzero}{non-zero\spc}
\newcommand {\seq}{\mathchoice {\otimes}{\otimes}{{\pmb{\otimes}}}{\otimes}}
\newcommand {\pt}{pt}
\DeclareSymbolFont{mysymbols}{OMS}{cmsy}{m}{n}
\DeclareMathSymbol {\OO}{\mathalpha}{mysymbols}{`O}
\DeclareMathSymbol {\cc}{\mathalpha}{mysymbols}{`C}
\DeclareMathSymbol {\calT}{\mathalpha}{mysymbols}{`T}
\DeclareMathSymbol {\calD}{\mathalpha}{mysymbols}{`D}
\DeclareMathSymbol {\calB}{\mathalpha}{mysymbols}{`B}
\DeclareMathSymbol {\calL}{\mathalpha}{mysymbols}{`L}
\DeclareMathSymbol {\calH}{\mathalpha}{mysymbols}{`H}
\DeclareMathSymbol {\calE}{\mathalpha}{mysymbols}{`E}
\DeclareMathSymbol {\calI}{\mathalpha}{mysymbols}{`I}
\DeclareMathSymbol {\calJ}{\mathalpha}{mysymbols}{`J}
\DeclareMathSymbol {\calP}{\mathalpha}{mysymbols}{`P}
\DeclareMathSymbol {\MM}{\mathalpha}{mysymbols}{`M}
\newcommand {\EExt}{\calE xt}
\newcommand {\eqn}[4]{{\calE}_{#1}(#2 \;;\;#3\;|\;#4)}
\newcommand {\ZZ}{{\mathbb Z}}
\newcommand {\PP}{{\mathbb P}}
\newcommand {\bP}{\tilde \PP}
\newcommand {\QQ}{{\mathbb Q}}
\newcommand {\RR}{{\mathbb R}}
\newcommand {\CC}{{\mathbb C}}
\newcommand {\HH}{{\mathbb H}}
\newcommand {\NN}{{\mathbb N}}
\newcommand {\df}[1]{\textbf {#1}}
\newcommand {\mdf}[1]{{\pmb {#1}}}
\newcommand {\dhz}{\partial_{H_2}}
\newcommand {\dhd}{\partial_{H_3}}
\newcommand {\dhv}{\partial_{H_4}}
\newcommand {\dmd}{\partial_{M_3}}
\newcommand {\dc}{\partial_{C}}
\newcommand {\isom}{\cong}
\renewcommand {\labelenumi}{(\roman{enumi})}
\renewcommand {\amalg}{\stackrel {{\scriptscriptstyle \bullet}}{\cup}}
\renewcommand {\emph}[1]{{\textsl {#1}}}
\makeatother
\newcommand {\xydiag}[1]{\[ \xymatrix @M=5pt {#1} \]}

\theoremstyle {plain}
\theorembodyfont {\normalfont\slshape}
\newtheorem {theorem}{Theorem}[section]
\newtheorem {lemma}[theorem]{Lemma}
\newtheorem {algorithm}[theorem]{Algorithm}
\newtheorem {proposition}[theorem]{Proposition}
\newtheorem {corollary}[theorem]{Corollary}
\newtheorem {definition}[theorem]{Definition}
\newtheorem {example}[theorem]{Example}
\newtheorem {remark}[theorem]{Remark}
\newenvironment {proof}{\textbf {Proof }}{\hfill $ \Box $}

\textheight 23cm
\topmargin -5mm
\textwidth 145mm
\oddsidemargin 8mm
\evensidemargin 1mm
\parindent 0mm
\parskip 0.8ex plus0.3ex minus 0.2ex
\renewcommand {\baselinestretch}{1.1}
\pagestyle {headings}

